Imaging of X-ray Pairs in a Spontaneous Parametric Down-Conversion Process

Spontaneous parametric down-conversion is a vital method for generating correlated photon pairs in the visible and near-infrared spectral regions; however, its extension to X-ray frequencies has faced substantial barriers. Here, we present an advancement in correlated X-ray pair generation and detection by employing a two-dimensional pixelated detector to obtain the first direct image of the pair distribution. Our study explores and directly visualizes the down-conversion process, revealing the characteristic ring structure of coincident photon pairs and demonstrating robust spatial correlations. A significant finding is the observation of energy anti-correlation, achieved at an unprecedented rate of approximately 4,100 pairs/hour, far exceeding previous reports in the literature. We believe these results represent a significant leap in X-ray quantum imaging, unlocking the potential for enhanced imaging of biological materials with reduced doses and broadening the applicability of X-ray quantum optical technologies.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


